Can Large Language Models Really Improve by Self-critiquing Their Own Plans?

There have been widespread claims about Large Language Models (LLMs) being able to successfully verify or self-critique their candidate solutions in reasoning problems in an iterative mode. Intrigued by those claims, in this paper we set out to investigate the verification/self-critiquing abilities of large language models in the context of planning. We evaluate a planning system that employs LLMs for both plan generation and verification. We assess the verifier LLM's performance against ground-truth verification, the impact of self-critiquing on plan generation, and the influence of varying feedback levels on system performance. Using GPT-4, a state-of-the-art LLM, for both generation and verification, our findings reveal that self-critiquing appears to diminish plan generation performance, especially when compared to systems with external, sound verifiers and the LLM verifiers in that system produce a notable number of false positives, compromising the system's reliability. Additionally, the nature of feedback, whether binary or detailed, showed minimal impact on plan generation. Collectively, our results cast doubt on the effectiveness of LLMs in a self-critiquing, iterative framework for planning tasks.

==> prompts/bp_all.tex <==
====GPT-4 Plan====
unstack the yellow block from the red block
put down the yellow block
unstack the red block from the orange block
put down the red block
pick up the yellow block
stack the yellow block on top of the orange block
pick up the red block
stack the red block on top of the blue block
====== Verification and Feedback ========
The above plan is invalid.
There are unsatisfied preconditions.
The following action at step 8 has an unmet precondition:
stack the red block on top of the blue block
The unmet precondition is:
the blue block is clear The following action at step 9 has unmet preconditions:
unstack the blue block from on top of the red block
The unmet preconditions are:
the blue block is clear and the blue block is on top of the red block

==> prompts/bp_binary.tex <==
====GPT-4 Plan====
unstack the yellow block from the red block
put down the yellow block
unstack the red block from the orange block
put down the red block
pick up the yellow block
stack the yellow block on top of the orange block
pick up the red block
stack the red block on top of the blue block
====== Verification and Feedback ========
The above plan is invalid.


==> prompts/bp_example.tex <==
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.
Once you stack a block on top of a second block, the second block is no longer clear.

[STATEMENT]
As initial conditions I have that, the orange block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the red block, the orange block is on top of the blue block, the red block is on the table and the yellow block is on the table.
My goal is to have that the blue block is on top of the red block and the yellow block is on top of the orange block.

My plan is as follows:

[PLAN]
pick up the yellow block
stack the yellow block on top of the orange block
[PLAN END]

[STATEMENT]
As initial conditions I have that, the yellow block is clear, the hand is empty, the red block is on top of the orange block, the orange block is on top of the blue block, the yellow block is on top of the red block and the blue block is on the table.
My goal is to have that the red block is on top of the blue block and the yellow block is on top of the orange block.

My plan is as follows:

[PLAN]

==> prompts/bp_val.tex <==
====GPT-4 Plan====
unstack the yellow block from the red block
put down the yellow block
unstack the red block from the orange block
put down the red block
pick up the yellow block
stack the yellow block on top of the orange block
pick up the red block
stack the red block on top of the blue block
====== Verification and Feedback ========
The above plan is invalid.
The following action at step 8 has an unmet precondition:
stack the red block on top of the blue block
The unmet precondition is:
the blue block is clear

==> prompts/plan_gen.tex <==
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.

[STATEMENT]
As initial conditions I have that, the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table.
My goal is to have that the orange block is on top of the blue block.

My plan is as follows:

[PLAN]
unstack the blue block from on top of the orange block
put down the blue block
pick up the orange block
stack the orange block on top of the blue block
[PLAN END]

[STATEMENT]
As initial conditions I have that, the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table and the orange block is on the table.
My goal is to have that the orange block is on top of the red block.

My plan is as follows:

[PLAN]

==> prompts/plan_ver.tex <==
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.
Once you stack a block on top of a second block, the second block is no longer clear.

[STATEMENT]
As initial conditions I have that, the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table and the orange block is on the table.
My goal is to have that the orange block is on top of the red block. 
My plan is as follows:

[PLAN]
unstack the yellow block from on top of the orange block
put down the yellow block
unstack the red block from on top of the blue block
put down the red block
pick up the orange block
stack the orange block on top of the red block
[PLAN END]

Verify whether the above plan is valid. If it is valid, please say "Plan is valid." and nothing else. If it is invalid, please say "Plan is invalid." and then provide feedback on why the plan fails.
